Constrained Reinforcement Learning for Robotics via Scenario-Based Programming

Deep reinforcement learning (DRL) has achieved groundbreaking successes in a wide variety of robotic applications. A natural consequence is the adoption of this paradigm for safety-critical tasks, where human safety and expensive hardware can be involved. In this context, it is crucial to optimize the performance of DRL-based agents while providing guarantees about their behavior. This paper presents a novel technique for incorporating domain-expert knowledge into a constrained DRL training loop. Our technique exploits the scenario-based programming paradigm, which is designed to allow specifying such knowledge in a simple and intuitive way. We validated our method on the popular robotic mapless navigation problem, in simulation, and on the actual platform. Our experiments demonstrate that using our approach to leverage expert knowledge dramatically improves the safety and the performance of the agent.

==> sections/backgroung_backup.tex <==
\section{Background}
\label{sec:background}
%\subsection{Neural Network and Reinforcement Learning}

Deep neural networks (DNNs)~\citep{GoBeCo16} are computational models represented by multiple-layer directed graphs. 
%\raz{Guy - I have changed \cite to \citep }
The network computes a single value, or a classification label, based on assigning fixed inputs to the first layer of the graph and propagating the computations through the subsequent layers, until reaching the final layer and returning the outputs to the user. 
Each layer computes values that depend on the previous layer's computations and the current layer's \textit{type}. 
For example, in the common \emph{rectified linear unit} (\emph{ReLU}) layer,
each node $y$ computes the value $y=\relu{}(x)=\max(0,x)$, based
on a single node $x$ from the preceding layer to which it is
connected. In addition, DNNs are abundant with \emph{weighted sum} layers, in which each neuron is computed as an affine transformation of the neurons from the preceding layer.
The DRL systems which are the subject matter of this work consist solely of weighted sum and \relu{} layers, although our approach is also suitable for DNNs with other layer types.

Fig.~\ref{fig:toyDnn} depicts a simple example of a DNN. For input
$V_1=[1, -1]^T$, the second (weighted sum) layer computes $V_2=[1,-4]^T$. Next, the \relu{} functions are applied in the third layer, 
resulting to $V_3=[1,0]^T$. Finally, the network's outputs a single weighted sum value: $V_4=[2]$.


\begin{figure}[htp]
	%\begin{wrapfigure}[8]{r}{6.0cm}
	\begin{center}
		\scalebox{0.8} {
			\def\layersep{2.0cm}
			\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node 
				distance=\layersep,font=\footnotesize]
				
				\node[input neuron] (I-1) at (0,-1) {$v^1_1$};
				\node[input neuron] (I-2) at (0,-2.5) {$v^2_1$};
				
				\node[hidden neuron] (H-1) at (\layersep,-1) {$v^1_2$};
				\node[hidden neuron] (H-2) at (\layersep,-2.5) {$v^2_2$};
				
				\node[hidden neuron] (H-3) at (2*\layersep,-1) {$v^1_3$};
				\node[hidden neuron] (H-4) at (2*\layersep,-2.5) {$v^2_3$};
				
				\node[output neuron] at (3*\layersep, -1.75) (O-1) {$v^1_4$};
				
				% Connect every node in the hidden layer with the output layer 
				\draw[nnedge] (I-1) --node[above] {$3$} (H-1);
				\draw[nnedge] (I-1) --node[above, pos=0.3] {$\ -1$} (H-2);
				\draw[nnedge] (I-2) --node[below, pos=0.3] {$5$} (H-1);
				\draw[nnedge] (I-2) --node[below] {$1$} (H-2);
				
				\draw[nnedge] (H-1) --node[above] {$\relu$} (H-3);
				\draw[nnedge] (H-2) --node[below] {$\relu$} (H-4);
				
				\draw[nnedge] (H-3) --node[above] {$2$} (O-1);
				\draw[nnedge] (H-4) --node[below] {$-1$} (O-1);
				
				
				% Biases
				\node[below=0.05cm of H-1] (b1) {$+3$};
				\node[below=0.05cm of H-2] (b2) {$-2$};
				
				% Annotate the layers
				\node[annot,above of=H-1, node distance=0.8cm] (hl1) {Weighted 
					sum};
				\node[annot,above of=H-3, node distance=0.8cm] (hl2) {ReLU };
				\node[annot,left of=hl1] {Input };
				\node[annot,right of=hl2] {Output };
			\end{tikzpicture}
		}
		\captionsetup{size=small}
		\captionof{figure}{A toy DNN.}
		\label{fig:toyDnn}
	\end{center}
	%\end{wrapfigure}
\end{figure}



\textbf{Deep Reinforcement Learning:}  Deep reinforcement
  learning (DRL)~\citep{Li17} is a specific setting used for training DNNs, in which the DNN is trained to serve as an \textit{agent} used to learn a \emph{policy} $\pi$, mapping each possible observed \emph{environment state} $s$ to an \emph{action} $a$. 
  During the DRL training phase, a matching \textit{reward} $r_t$ is presented to the agent, at each discrete time-step $t\in{0,1,2...}$. Each reward is based on the action $a_t$  performed by the agent on time-step $t$. DRL training algorithms leverage the reward in various ways, in order to strategically optimize the agent's parameters during training. We note that DRL-trained DNNs have, in general, the same DNN architecture described above; and that the uniquness of the DRL paradigm lies in the training process, which aims to generate a DNN that computes a policy $\pi$ maximizing the \textit{expected
  cumulative discounted reward} 
  $R_t=\mathbb{E}\big[\sum_{t}\gamma^{t}\cdot r_t\big]$. 
  The \textit{discount factor}, $\gamma \in \big[0,1\big]$, is a hyperparmeter that controls the impact of past decisions on the total expected reward.

\subsection{PPO and Lagrangian-PPO}
Historically, reinforcement learning algorithms are subdivided into two major categories: \textit{Value-Based}~\citep{MnKaSiGrAnWiRi13} and \textit{Policy Gradient}~\citep{SuBa18}. In addition, to combine the strengths of both these approaches, the \textit{Actor-Critic}~\citep{LiHuPr15} methods have been introduced. In the context of the policy gradient strategies, one of the first successful implementations of this last approach is the Advantage Actor-Critic (A2C)~\citep{MhBaMi16} algorithm. The key contribution is to replace the return with a new objective for the optimization, which intuitively represents the expected reward advantage of selecting a specific action $a$ with respect to the estimated value of the current state. The gradient of the objective function, derived from the \textit{policy gradient theorem} becomes:
\begin{equation}
    \nabla_\theta J_R(\pi)=\mathbb{E}_{\tau\sim\pi} \big[\sum_{t}^T \nabla \log\pi_\theta(a_t | s_t ) A(s_t, a_t)\big]
\label{eq:background:A2C}
\end{equation}

Proximal Policy Optimization (PPO) is considered a state of the art algorithm for reinforcement learning~\citep{ShWoDh17}, and can be viewed as an evolution of A2C and, in general, of the policy gradient methods. Intuitively, the key characteristic of PPO is to limit the step size between two consecutive updates to avoid changes that can drastically modify the behavior~\citep{ScLeAbJo15}.
More formally, the objective function of PPO is the following:
\begin{equation}
    J_{R}(\pi) = \mathbb{E}\big[min( r(\theta)A(s, a), clip(r(\theta), 1+\epsilon, 1-\epsilon)A(s, a)) \big] \quad r(\theta)=\frac{\pi_\theta(a | s)}{\pi_\theta^{old}(a | s)}
\label{eq:background:ppo}
\end{equation}
where $A(s, a)$ is the advantage of taking the action $s$ in the state $s$ and $r(\theta)$ is the ratio between the probability of taking the action $a$ between the current and the updated policy. 


As explained in the recent paper from~\citet{SiSiPr21}, it is common to believe that the \textit{reward is enough} to describe any kind of desired behavior. However, especially in \textit{safety-critical tasks} the concept of optimality goes beyond the simple maximization of the return but involves some hard constraints the agent must respect to guarantee different forms of safety. 
In this direction, an alternative framework for sequential decision making is the \textit{Constrained Markov Decision Process (CMDP)}.
A CMDP is a markov decision process enriched with an additional signal, the \textit{cost function}, defined as $C: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$, whose expectation must remain below a given threshold $d \in \mathbb{R}$ (notice that CMDP supports multiple constraints and cost functions, in that case we denote the cost function and the threshold with $C_k$ and $d_k$). The set of \textit{valid} policies for a CMDP is therefore defined as:
\begin{equation}
    \Pi_\mathcal{C} := \{\pi \in \Pi : J_{C_k}(\pi) \leq d_k,~\forall k\}
\label{eq:background:valid_cmdp}
\end{equation}
\noindent where $J_{C_k}(\pi)$ is the expected sum of the $k-th$ cost function and $d_k$ is the corresponding threshold. Intuitively, the objective is to find a function that respects the constraints (i.e., is \textit{valid}) while also maximize the expectation of the reward. An \textit{optimal} policy for a CMDP is formally defined as:
% \raz{Something is wrong with the armax cmd below here}
\begin{equation}
    \pi^*= \argmax_{\pi \in \Pi_\mathcal{C}} J_{r}(\pi)
\label{eq:background:optimal_cmdp}
\end{equation}
\noindent where $J_{C_k}(\pi)$ is the reward objective function.

A natural way to encode constraints in a classical optimization problem is through by using \textit{Lagrange multipliers}. Specifically, various methods in the constrained reinforcement learning domain exploit the Lagrangian duality~\citet{RaAcAm19}, to transform the problem into the corresponding dual unconstrained version. The optimization problem can then be encoded as follows:
\begin{equation}
   J(\theta) = \min_\pi \max_{\lambda \geq 0} \mathcal{L}(\pi, \lambda) = \min_\pi \max_{\lambda \geq 0} J_R(\pi) - \sum_K \lambda_k(J_{C_k}(\pi) - d_k)
\label{eq:background:lagrangian}
\end{equation}

Crucially, the optimization of the function $J(\theta)$ can be carried out by applying any \textit{policy gradient} algorithm, a common implementation is based on PPO~\citet{ShWoDh17}. However, even if theoretically sound, the actual application of the Lagrangian version of PPO (i.e., \textit{Lagrangian-PPO}) has shown unstable results when applied to complex tasks~\citet{MaCoFa21b}. In Section \ref{sec:methods}, we show the implementation of our optimized version of the algorithm, which shows excellent results in our case study.
Moreover, we demonstrate that the CMDP is a flexible framework and Lagrangian-PPO can be used, not only to find policies that respect some hard constraints but also to inject human knowledge and behavioral requirements into the training loop. 

\subsection{Scenario-based programming}
Scenario-based programming
(SBM)~\citep{DaHa01,HaMa03} is a paradigm designed to support the development of reactive systems by 
incorporating a language that is close to how humans perceive and describe reactive system behavior, 
focusing on inter-object system-wide behaviors.
In SBM, a system is composed of objects called \emph{scenario objects}, 
each describes a single desired (or undesired) behavioral aspect of the system. 
This behavior is formalized and modeled as a sequence of events.
%%moved down A scenario-based model is fully executable: when it runs, all its scenario objects are executed in parallel to each other, in a synchronized fashion, resulting in cohesive system behavior.  The resulting execution  thus complies with the requirements and constraints of each of the participating scenario objects~\citep{HaMa03,HaMaWe12ACM}.

More specifically, each such SBM scenario object can be
regarded as a transition system, whose states are referred to as
\emph{synchronization points}. The scenario object transitions between
synchronization points according to the triggering of \emph{events} by
a global \emph{event selection mechanism}. At each synchronization
point, each of the scenario objects may declare events that it \emph{requests} and events that it
\emph{blocks}. These declarations encode desirable and undesirable (e.g., forbidden) actions, as seen from the perspective of the particular scenario object making those declarations.
Scenario objects can also declare events that they passively \emph{wait-for}, thus asking to be notified once these events are triggered.
After making its event declarations, e.g., events it \emph{requests}, \emph{blocks}, or \emph{waits-for}, the scenario object is
suspended until any of these events are triggered,
at which point the scenario resumes and may transition to another
synchronization point. 

A scenario-based model is fully executable: at execution time, all its scenario objects run
in parallel to each other, until they all reach a synchronization point. Then, the
declarations of all requested and blocked events are collected by the
event selection mechanism, which selects and triggers one of the
events requested by at least one scenario object and is
blocked by none. 
The resulting execution thus complies with the requirements and constraints of each of the
scenario objects of the model~\citep{HaMa03,HaMaWe12ACM}.


Fig.~\ref{fig:watertap} depicts a scenario-based model of a simple system that controls the temperature and water-level in a water tank, borrowed from~\citep{HaKaMaWe12}. 
Each of the scenario objects is shown as a transition system, with the nodes representing synchronization points. 
The transition edges are associated with the requested or waited-for events in the preceding node. 
The scenarios \emph{AddHotWater} and \emph{AddColdWater} repeatedly wait for \b{WaterLow}
events and then request three times the event \b{AddHot} or \b{AddCold}, respectively.  Since these six events may be triggered in any order by the event selection mechanism, a new scenario \emph{Stability} is added, with the purpose of keeping the water temperature more stable by enforcing the interleaving of \b{AddHot} and \b{AddCold} events, by alternately blocking them. The resulting execution trace is shown in the event log.

%The scenarios \j{AddHotWater} and \j{AddColdWater} repeatedly wait for \j{WaterLow} events and then request three times the event \j{AddHot} or \j{AddCold}, respectively.  Since these six events may be triggered in any order by the event selection mechanism, a new scenario \j{Stability} is added, with the purpose of keeping the water temperature more stable by enforcing the interleaving of \j{AddHot} and \j{AddCold} events, by alternately blocking them. The resulting execution trace is shown in the event log.
    
\raz{Davide, Guy - I tried to refresh the graphics of the Water Tap, but I can not get it compact enough.Not sure it is critical.}
%\begin{figure*}[htb]
%	\centering
%  \scalebox{0.7} {
%    \subfigure[AddHotWater]{\includegraphics[width=0.5\textwidth]{images/add-hot_A5_large font.pdf}
%    \label{fig:background:watertap_addhot}}
%    \subfigure[AddColdWater]{\includegraphics[width=0.5\textwidth]{images/add-coldA5_large font.pdf}
%        \label{fig:background:watertap_addcold}}
%    \subfigure[Stability]{\includegraphics[width=0.5\textwidth]{images/stabilityA5_large font.pdf}
%    \label{fig:background:watertap_stability}}
%\subfigure[EventLog]
%        {\includegraphics[width=0.3\textwidth]{images/logger_EnvelopSize_large font.pdf}
%    \label{fig:background:watertap_eventlog}}
%	}
%	\caption{(Inspired by~\citep{HaKaMaWe12}) A scenario-based model for controlling water-level and temperature.}
%	\label{fig:watertap_hide}
%\end{figure*} 

\begin{figure*}[htb]
	\centering
  \scalebox{0.7} {
	\includegraphics[width=0.8\textwidth]{images/WaterPump_new_alltogether.pdf}
	}
	\caption{(Inspired by~\citep{HaKaMaWe12}) A scenario-based model for controlling water-level and temperature.}
	\label{fig:watertap}
\end{figure*} 


    
%\newcommand{\request}{{\color{blue}request}}
%\newcommand{\waitfor}{{\color{green!50!black}wait for}}
%\newcommand{\blocking}{{\color{red}blocking}}
%\begin{figure}[tb]
%  \centering
%  \scalebox{0.85} {
%
%    \tikzstyle{box}=[draw,  text width=2cm,text centered,inner sep=3]
%    \tikzstyle{set}=[text centered, text width = 10em]
%
%    \begin{tikzpicture}[thick,auto,>=latex',line/.style ={draw, thick, -latex', shorten >=0pt}]
%
 %     \matrix(bts) [row sep=0.3cm,column sep=2cm]  {
%
%       \node (box1)  [box] {\waitfor{} \j{WaterLow}}; \\
%        \node (box2)  [box] {\request\ \j{AddHot}}; \\
%        \node (box3)  [box] {\request\ \j{AddHot}}; \\
%        \node (box4)  [box] {\request\ \j{AddHot}}; \\
%      };
%
 %     \node (title) [above=0.1cm of bts,box,draw=none] at ($(bts) + (-0.25cm,2.31cm)$)
 %     {\j{AddHotWater}};
%
 %     \begin{scope}[every path/.style=line]
 %       \path (box1)   -- (box2);
 %       \path (box2)   -- (box3);
 %       \path (box3)   -- (box4);
 %       \path (box4.east)   -- +(.25,0) |- (box1);
 %     \end{scope}
%
%
 %     \matrix(bts2) [right=.25cm of bts, row sep=0.3cm,column sep=2cm] {
 %       \node (box1)  [box] {\waitfor{} \j{WaterLow}}; \\
 %       \node (box2)  [box] {\request\ \j{AddCold}}; \\
 %       \node (box3)  [box] {\request\ \j{AddCold}}; \\
 %       \node (box4)  [box] {\request\ \j{AddCold}}; \\
 %     };
%
 %     \node (title) [above=0.1cm of bts2,box,draw=none] at ($(bts2) + (-0.25cm,2.31cm)$)
 %     {\j{AddColdWater}};
%

%      \begin{scope}[every path/.style=line]
%        \path (box1)   -- (box2);
%        \path (box2)   -- (box3);
%        \path (box3)   -- (box4);
%        \path (box4.east)   -- +(.25,0) |- (box1);
%      \end{scope}
%
%
%      \matrix(bts3) [right=.25cm of bts2, row sep=0.3cm,column sep=2cm] {
%        \node (box1)  [box] {\waitfor{}  \j{AddHot} while  \blocking\ \j{AddCold}}; \\
%        \node (box2)  [box] {\waitfor{}  \j{AddCold} while \blocking\ \j{AddHot}}; \\
%      };
%
%      \node (title) at (title-|bts3) [box,draw=none] {\j{Stability}};
%
%      \begin{scope}[every path/.style=line]
%        \path (box1)   -- (box2);
%        \path (box2.east)   -- +(.25,0) |- (box1);
%      \end{scope}
%
%      \node (log)  [right=.3cm of bts3,box,text width=2cm,fill=yellow!20] {
%        $\cdots$ \\
%        \j{WaterLow} \\
%        \j{AddHot}  \\
%        \j{AddCold} \\
%        \j{AddHot}  \\
%        \j{AddCold} \\
%        \j{AddHot}  \\
%        \j{AddCold} \\
%        $\cdots$ \\
%      };
%
%      \node (title2) at (title-|log)
%      [box,draw=none] {\j{Event Log}};
%    \end{tikzpicture}
%  }
%  \caption{(Borrowed from~\citep{HaKaMaWe12}) A scenario-based model for controlling water-level and temperature. }
%  \label{fig:watertap_hide}
%\end{figure}

\guyamir{I'm not sure we need the next paragraph.}
In practice, SBM is supported
in multiple textual and visual frameworks. Worthnoty examples
include the language of \emph{live sequence charts} (LSC), where SBM
concepts are applied to produce modal sequence
diagrams~\citep{DaHa01,HaMa03}; implementations in
various high-level languages, such as Java, C++, JavaScript, and Python (see, e.g.,~\citep{HaMaWe12ACM}); and various
domain-specific languages~\citep{GrGrKaMa16} and
extensions~\citep{HaKaMaSaWe20,KaMaSaWe19}.

A particularly useful aspect of SBM is that the resulting model is 
amenable to model checking, and facilitates compositional
verification~\citep{HaLaMaWe11BPMC,HaKaKaMaMiWe13,Ka13, HaKaMaWe15,KaBaHa15,HaKaLaMaWe15}. 
Hence, it is possible to use formal verification to ensure that a
scenario-based model satisfies various properties. 

A plethora of techniques support different extensions and usages of SBM:
A technique to execute scenario-based models in distributed
architectures~\citep{HaKaKaMaWeWi15,StGrGrHaKaMa18,StGrGrHaKaMa17,GrGrKaMaGlGuKo16,HaKaKa13},
to automatically repair these
models~\citep{HaKaMaWe14,HaKaMaWe12,Ka21}, and to augment them in
various ways, e.g., as part of the Wise Computing
initiative~\citep{HaKaMaMa18,MaArElGoKaLaMaShSzWeHa16,HaKaMaMa16,HaKaMaMa16b}.

SBM is an attractive choice for the incorporation of domain-specific knowledge
into a DRL agent training process, being formal, fully executable and support of incremental development ~\citep{GoMaMe12Spaghetti,AlArGoHa14CognitiveLoad}.
Moreover, the language it uses enables domain-specific experts to directly   
express their requirements specification as an SBM model.

%Indeed, using SBM to complement DRL was demonstrated in the past, although the focus
%so far has been on \emph{guarding} an already-trained DRL agent,
%rather than 
%affecting what the agent actually learns~\citep{katz2020guarded,katzElyasaf2021DLSBP}.


\subsection{Formal Verification of DNNs and DRLs}

A DNN verification algorithm receives the following fixed inputs~\citep{KaBaDiJuKo17}: a trained DNN $N$, a precondition $P$ on the DNN's inputs, which limits their possible assignments to inputs of interest; and a postcondition $Q$ on $N$'s output.
The inputs usually express some assumption the user has, regarding the environment (e.g., pixel values, for a DNN trained on images). In addition, the postconidtion typically encodes the \textit{negation} of the behavior we would like $N$ to exhibit on
all possible inputs that satisfy $P$.

Then, the verification algorithm search for an input $x'$ that satisfies the given preconditions (i.e.,  $P(x') \wedge Q(N(x'))$), and returns exactly one of the following outputs:
\begin{inparaenum}[(i)]
\item \sat, indicating the query is satisfiable. Due to the postcondition $Q$ encoding the negation of the required property, this result indicates that the wanted property is violated in some cases.
Modern verification engines also supply a concrete input $x'$ that satisfies the query, and hence, a valid input that triggers a bug, such as an incorrect classification.
\item \unsat, indicating that no for all $x_0$ inputs the negated property never holds, and thus --- proving that the original (wanted) property always holds.
\end{inparaenum}
 


For example, if we were interested in guaranteeing that
for all non-negative inputs $x=\langle v_1^1,v_1^2\rangle$
the DNN in Fig.~\ref{fig:toyDnn} always outputs a value strictly smaller than $40$; i.e., it holds that $N(x)=v_4^1 < 40$. This property is encoded as a verification query consisting of a precondition that restrict the inputs to the desired range, i.e.,
$P=(v_1^1 \geq 0) \wedge (v_1^2 \geq 0)$, and by setting $Q=(v_4^1\geq 40)$, which is the
\textit{negation} of the desired property. 
In this case, a sound verifier will return \sat, alongside a feasible
counterexample such as $x=\langle 2, 3\rangle$, which produces the output
$v_4^1=48 \geq\ 40$ when fed to the DNN. Hence, the property does not always hold.


Originally, the most DNN verification engines were designed the verify the correct behaviour of feed-forward
DNNs~\citep{ KaBaDiJuKo17, GeMiDrTsChVe18, WaPeWhYaJa18, LyKoKoWoLiDa20, HuKwWaWu17}. However, in recent years,
the verification community has also designed verification methods tailored for DRL systems~\citep{CoMaFa21, BaGiPa21, ElKaKaSc21, AmScKa21, AmCoYeMaHaFaKa22}. These methods include techniques for encoding multiple invocations of the agent in questions, when interacting with a 
typically reactive environment over multiple time-steps.


%\guyamir{Davide - can you try to fix some of the background sections I wrote and don't appear? I think it has something to do with the citations but not sure}
